Counterfactual Explanations for Arbitrary Regression Models

We present a new method for counterfactual explanations (CFEs) based on Bayesian optimisation that applies to both classification and regression models. Our method is a globally convergent search algorithm with support for arbitrary regression models and constraints like feature sparsity and actionable recourse, and furthermore can answer multiple counterfactual questions in parallel while learning from previous queries. We formulate CFE search for regression models in a rigorous mathematical framework using differentiable potentials, which resolves robustness issues in threshold-based objectives. We prove that in this framework, (a) verifying the existence of counterfactuals is NP-complete; and (b) that finding instances using such potentials is CLS-complete. We describe a unified algorithm for CFEs using a specialised acquisition function that composes both expected improvement and an exponential-polynomial (EP) family with desirable properties. Our evaluation on real-world benchmark domains demonstrate high sample-efficiency and precision.

==> attic.tex <==
\section{Orthogonal polynomials and numerical quadrature}

\paragraph{Gaussians and Hermite polynomials}

For a Gaussian kernel $\phi(x) = \exp\left(-\frac 1 2 x^2\right)$ over the entire real line $S = \mathbb R = (-\infty, \infty)$, the natural orthogonal polynomials are the (probabilist's) Hermite polynomials

\[
\He_n = (-1)^n \phi(x) (\frac d {dx})^n \phi(x)
\]

which have the nice orthogonal property

\[
\int_S \He_m (x) \He_n (x) \phi(x) dx = \sqrt{2\pi} n! \delta_{mn} 
\]

There some nice closed form expressions like Rodrigues's formula

\[
\He_n(x) = (x - d/dx)^n \cdot 1
\]

but the most useful property of orthogonal polynomials is the three-term recurrence

\[
\He_n(x) = x \He_{n-1}(x) - \He^\prime_{n-1}(x) = x \He_{n-1}(x) - (n-1) \He^\prime_{n-2}(x) 
\]

What is less useful is the explicit power series expansion of an Hermite polynomial

\[
\He_n(x) = n! \sum_{m=0}^{\floor*{\frac n 2}} \frac{x^{n-2m}} {2^m}
\]

While you can calculate this formula in closed form, it's not very useful in practice.
However, the useful concept to abstract away is that the coefficients of this expansion can be collected into some triangular matrix $\{A_{m,n}\}$,
which now fully describes the \textit{change of basis} from the monomials $M = \{1, x, x^2, ...\}$ to the Hermite polynomials.

Formally, this is just the linear system of equations

\[
\He = A M
\]

There's also a linear algebra aspect to this observation.
Grouping the recurrences into a matrix $T$, this matrix now describes the
endomorphism mapping Hermite polynomials to themselves:

\[
\He_n(x) = x \He_{n-1}(x) - \He^\prime_{n-1}(x) = x \He_{n-1}(x) - (n-1) \He^\prime_{n-2}(x) 
\]

\[
T \He = 
\begin{pmatrix}
0 & 1 \\
1 & 0 & 1 \\
  & 2 & 0 & 1 \\
  &   & 3 & 0 & 1 \\
  &   & \ddots
\end{pmatrix}
= x \He
\]

It turns out to be more convenient to write down the recurrence in symmetric form, which is called the Jacobi matrix $J$:

\[
\sqrt{n} \He_{n+1} (x) + \sqrt{n} \He_{n-1}(x) = x \He_{n}(x) 
\]

\begin{equation}
J \He = 
\begin{pmatrix}
0 & 1 \\
1 & 0 & \sqrt 2 \\
  & \sqrt 2 & 0 & \sqrt 3 \\
  &   & \sqrt 3 & 0 & 2 \\
  &   & & \ddots
\end{pmatrix}
= x \He
\label{eq:jacobi}
\end{equation}

In this manner, you can see that all orthogonal polynomials form alternative basis to represent all polynomials $\sum_n a_n x^n$!
It's equivalent to define polynomials as the set of all functions of the form $\sum_n a_n \He_n(x)$, for example.

This construction of orthogonal polynomials can be very general.

For example, given a finite interval $S = [-1, 1]$ and the trivial kernel $\phi(x) = 1$,
the natural orthogonal polynomials are the Legendre polynomials

\[
P_n = \frac 1 {2^n n!} \left(\frac d {dx}\right)^n (x^2 - 1)^n
\]

which have the orthogonal property

\[
\int_S P_m (x) P_n (x)  dx = \frac 2 {2n+1} \delta_{mn} 
\]

and the three-term recurrence

\[
n P_n (x) = (2n+1) x P_{n-1}(x) - (n-1) P_{n-2}(x) 
\]

\paragraph{General construction}
Why is the three-term recurrence so important?
All orthogonal polynomials have a 3-term recurrence of the form $p_{n+1}(x) = (x + c_n) p_n(x) + d_n p_{n-1}(x)$
for some constants $c_n$ and $d_n$.
The converse is also true. Favard's theorem says that polynomials with a 3-term recurrence of the form
$p_{n+1}(x) = (x + c_n) p_n(x) + d_n p_{n-1}(x)$ are orthogonal polynomials

The explicit closed form expressions for the orthogonal polynomials can look mysterious at first,
but these are for the most part derived ex poste. What really matters is discovering the recurrence.
You can use the Gram-Schmidt procedure to construction for orthogonal polynomials for any weight function,
given only the inner product structure
\[
\left\langle f \middle\vert g \right\rangle = \int_S f(x) g(x) \phi(x) dx
\]
Set $p_0(x) = 1$ and construct $p_1(x) = x + c$ in the monomial basis.
Solve for the coefficient $c$ using the orthogonality constraint $\left\langle p_1 \middle\vert p_0 \right\rangle = 0$.
By induction, you can have the Gram-Schmidt result
\[
p_n(x) = x^n - \sum_{k=0}^{n-1} \frac {\left\langle x^n \middle\vert p_k \right\rangle} {\left\langle p_k \middle\vert p_k \right\rangle} p_k(x)
\]

\paragraph{Generalizations}

You can also use this construction for any inner product structure where the measure is not $\phi(x) dx$, but discrete, or even a mixture of discrete and continuous measures.
There are also generalizations to multivariate polynomials known as the Macdonald polynomials, which are symmetric under permutations of their arguments.

\paragraph{Quadrature}

Now for why this matters for numerical integration. Suppose we want to calculate some integral

\[
\int_S \phi(x) f(x) dx \approx \sum^n_{i=1} w_i f(x_i)
\]

The standard thing to do is something like the rectangle rule like in the definition of the Riemann sum: split the finite interval $S$ into $n$ equal pieces $(x_1, ..., x_n)$. Each such point is called a quadrature point or node. However, we can do better to approximate this integral numerically.
Take $S = [-1, 1]$, $\phi(x) = 1$, $x_i$ to be the roots of $P_n(x) = 0$ with corresponding weights $w_i = 2/((1-x_i)^2 (P^\prime_n(x_i))^2)$.
This set of weights and nodes defines what is known as Gaussian quadrature, or Gauss-Legendre quadrature.

Why is this such a big deal?
One major result is that for any polynomial of degree $n$, $p_n(x) = \sum_k a_k x^k$, $a_n \ne 0$, $a_{n-1} \ne 0$,
such that
\[
\int_S \phi(x) x^k p_n(x) dx = 0
\]
for all $k=0,1,...n-1$, then there exist nodes $x_i$ that are roots of $p_n(x) = 0$ with corresponding positive weights
\[
w_i = \frac {a_n} {a_n-1} \frac{\int_S \phi(x) p_{n-1}(x)^2 dx}{p^\prime_n(x_i) p_{n-1}(x_i)}
\]
that make the quadrature scheme $(x_i, w_i)$ exact for all polynomials of up degree $2n-1$, i.e., $\sum_{i=1}^n w_i p_m(x_i) = 0$
for all $m < 2n$. (This result can be derived by writing $x^n$ in the $p_n$ basis and then using the Christoffel--Darboux identity.) 

Furthermore, there is a Taylor-like error theorem that states that for an integrand $f$ with at least $2n$ continuous derivatives,
the quadrature error is

\[
\int_S \phi(x) f(x) dx - \sum_{i=1}^n w_i f(x_i) = \frac {f^{(2n)} (\xi)}{(2n)!} \int_S \phi(x) p_n^2(x) dx
\]
for some $\xi \in S$. (This formula for the quadrature error is at best a theoretical tool since it doesn't tell you how to find $\xi$.)

So how do we derive the quadrature rule $(x_i, w_i)$?
The standard way is the Golub--Welsch algorithm, which simply
notes that if you want weights that are independent of coordinate $x$,
then what you have is an eigenproblem for $J$ in \eqref{eq:jacobi}!
The nodes $x_i$ are the eigenvalues
and the weights $w_i$ are the components of the eigenvector
corresponding to the largest eigenvalue.
By the Perron--Frobenius theorem, this eigenvector of a positive matrix
must have all positive entries. Thus all weights $w_i$ are strictly positive.
Furthermore, it turns out that there is an $O(n^2)$ way to solve the
eigenproblem for a symmetric tridiagonal matrix (and is in fact part of
the standard algorithm for diagonalizing symmetric / Hermitian matrices).

